Semantic GUI Scene Learning and Video Alignment for Detecting Duplicate Video-based Bug Reports

Video-based bug reports are increasingly being used to document bugs for programs centered around a graphical user interface (GUI). However, developing automated techniques to manage video-based reports is challenging as it requires identifying and understanding often nuanced visual patterns that capture key information about a reported bug. In this paper, we aim to overcome these challenges by advancing the bug report management task of duplicate detection for video-based reports. To this end, we introduce a new approach, called JANUS, that adapts the scene-learning capabilities of vision transformers to capture subtle visual and textual patterns that manifest on app UI screens - which is key to differentiating between similar screens for accurate duplicate report detection. JANUS also makes use of a video alignment technique capable of adaptive weighting of video frames to account for typical bug manifestation patterns. In a comprehensive evaluation on a benchmark containing 7,290 duplicate detection tasks derived from 270 video-based bug reports from 90 Android app bugs, the best configuration of our approach achieves an overall mRR/mAP of 89.8%/84.7%, and for the large majority of duplicate detection tasks, outperforms prior work by around 9% to a statistically significant degree. Finally, we qualitatively illustrate how the scene-learning capabilities provided by Janus benefits its performance.

==> macros.tex <==
\makeatletter

\newcommand{\toolname}{{\sc Janus}\xspace}
\newcommand{\toolnames}{{\sc Janus'}\xspace}
\newcommand{\toolnametxt}{{\sc $Janus_{txt}$}\xspace}
\newcommand{\toolnamevis}{{\sc $Janus_{vis}$}\xspace}
\newcommand{\toolnamelong}{{\sc \textbf{J}uxt\textbf{A}positio\textbf{N} of vis\textbf{U}al and textual modalitie\textbf{S}}\xspace}


\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	
% \newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
% \newcommand{\chapref}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\appref}[1]{Appendix~\ref{#1}\xspace}
% \newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\listref}[1]{Listing~\ref{#1}\xspace}
\newcommand{\equaref}[1]{Equation~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}


\newcommand\os[1]{{\color{violet} \nb{OSCAR}{#1}}}
\newcommand\yanfu[1]{{\color{red} \nb{YANFU}{#1}}}
\newcommand\nathan[1]{{\color{olive}\nb{NATHAN}{#1}}}
\newcommand\KEVIN[1]{{\color{blue}\nb{KEVIN}{#1}}}
\newcommand\denys[1]{{\color{orange}\nb{DENYS}{#1}}}

%\newcommand\NEW[1]{\nb{NEW}{#1}}
\newcommand\re{{\color{red} [REFs]}}
\newcommand\NEW[1]{{\color{black} #1}}
\newcommand\NEWR[1]{{\color{black} #1}}
\newcommand\NEWEST[1]{{\color{black} #1}}

\newcommand{\tango}{{\textsc{Tango}}\xspace}
\newcommand{\tangos}{{\textsc{Tango}'s}\xspace}
\newcommand{\tangot}{{\sc Tango$_{txt}$}\xspace}
\newcommand{\tangov}{{\sc Tango$_{vis}$}\xspace}
\newcommand{\tangoc}{{\sc Tango$_{comb}$}\xspace}
\newcommand{\tangovs}{{\sc Tango$_{vis}$'s}\xspace}

\newcommand{\approach}{{\textsc{Janus}}\xspace}
\newcommand{\ap}{\approach}
\newcommand{\aps}{{\textsc{Janus}'s}\xspace}

\newcommand{\janust}{{\sc Janus$_{txt}$}\xspace}
\newcommand{\janusv}{{\sc Janus$_{vis}$}\xspace}
\newcommand{\janusc}{{\sc Janus$_{comb}$}\xspace}

\newcommand{\janusts}{{\sc Janus$_{txt}$'s}\xspace}
\newcommand{\janusvs}{{\sc Janus$_{vis}$'s}\xspace}

\newcommand{\januss}{{\sc Janus$_{seq}$}\xspace}
\newcommand{\janusss}{{\sc Janus$_{seq}$'s}\xspace}

\newcommand{\janussv}{{\sc Janus$_{seq-v}$}\xspace}
\newcommand{\janusst}{{\sc Janus$_{seq-t}$}\xspace}

\newcommand{\janussvs}{{\sc Janus$_{seq-v}$'s}\xspace}
\newcommand{\janussts}{{\sc Janus$_{seq-t}$'s}\xspace}

\newcommand{\apt}{\janust}
\newcommand{\apv}{\janusv}

\newcommand{\apts}{\janusts}
\newcommand{\apvs}{\janusvs}


\newcommand{\apc}{\janusc}
\newcommand{\apss}{\januss}
\newcommand{\apsv}{\janussv}
\newcommand{\apst}{\janusst}
\newcommand{\apsvs}{\janussvs}
\newcommand{\apsts}{\janussts}

\newcommand{\apsss}{\janusss}

\def\signed#1{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil\sl#1
    \parfillskip=0pt \finalhyphendemerits=0 \par}}

\newcolumntype{?}{!{\vrule width 1pt}}
